QFix: Diagnosing errors through query histories

Data-driven applications rely on the correctness of their data to function properly and effectively. Errors in data can be incredibly costly and disruptive, leading to loss of revenue, incorrect conclusions, and misguided policy decisions. While data cleaning tools can purge datasets of many errors before the data is used, applications and users interacting with the data can introduce new errors. Subsequent valid updates can obscure these errors and propagate them through the dataset causing more discrepancies. Even when some of these discrepancies are discovered, they are often corrected superficially, on a case-by-case basis, further obscuring the true underlying cause, and making detection of the remaining errors harder. In this paper, we propose QFix, a framework that derives explanations and repairs for discrepancies in relational data, by analyzing the effect of queries that operated on the data and identifying potential mistakes in those queries. QFix is flexible, handling scenarios where only a subset of the true discrepancies is known, and robust to different types of update workloads. We make four important contributions: (a) we formalize the problem of diagnosing the causes of data errors based on the queries that operated on and introduced errors to a dataset; (b) we develop exact methods for deriving diagnoses and fixes for identified errors using state-of-the-art tools; (c) we present several optimization techniques that improve our basic approach without compromising accuracy, and (d) we leverage a tradeoff between accuracy and performance to scale diagnosis to large datasets and query logs, while achieving near-optimal results. We demonstrate the effectiveness of QFix through extensive evaluation over benchmark and synthetic data.

==> content/xx-conclusions.tex <==

\section{Conclusions}


==> content/xx-decisiontree.tex <==

\subsection{A plausible (but bad) alternative}
\label{sec:dt}


The MIP models generated by \sys can grow large as the sizes of the
data and the log increase. However, modeling all present constraints
from the beginning to the end of the log is necessary; in this
section, we examine alternative, simpler models that process a single
query at a time, and demonstrate why they are insufficient.

\smallskip
\noindent
\textbf{WHERE repairs through classification:}
The \texttt{WHERE} clause of an update query is equivalent to a
rule-based binary classifier that splits tuples into two groups:
(1)~tuples that satisfy the conditions in the \texttt{WHERE} clause
and (2)~tuples that do not. A mistake in a query predicate can then
result in misclassification: some tuples get classified into the wrong
group, which in turn translates to errors in the data. Therefore,
repairing the mistake corresponds to repairing the imprecise
classification. This works as follows: For an incorrect query $q$, let
$D_0$ be the database state before $q$, and $D_1^*$ the \emph{correct}
database state that should result after $q$.
We use each tuple $t \in D_0$ as an element in the input training data
for the classifier where the values (of each attribute) of $t$ define
the feature vector and the label for $t$:
	\[
    label(t)= 
    \begin{cases}
    true ,& D_0.t \neq D_1^*.t\\
    false,              & \text{otherwise}
    \end{cases}
\]
We then train a classifier, such as decision trees \cite{???} to learn
the correct classification rules rules for the \texttt{WHERE} clause.


\smallskip
\noindent
\textbf{SET repairs:}
After repairing the \texttt{WHERE} clause through learning a
rule-based classifier, some complaints may still persist. This
indicates a possible error in the \texttt{SET} clause. The errors can
be modeled and solved by constructing a simple linear system of
equations: For each expression in the \texttt{SET} clause we create a
linear equation, using unknown variables to represent any parameters
in the \texttt{SET} expression. Solving for these variables then
provides a repair for the \texttt{SET} expression.


\smallskip
\noindent
\textbf{Why it does not work:}
The na\"ive approach that we just described is heuristic in nature. It
is simple and fast, but it can only process a single incorrect query.
This results in several shortcomings that make it insufficient in
practice:
\begin{itemize}[itemsep=1pt, leftmargin=5mm]
    
\item In principle, one could attempt to apply this technique to the
entire log one-query-at-a-time. However, this is not possible in
practice: to learn a classifier on the \texttt{WHERE} clause of query
$q_i$, one needs to know the correct classification output, which
corresponds to $D_i^*$. Unfortunately, even with a complete complaint
set, which can derive the correct database $D_n^*$, there is no
obvious way to ``rollback'' this state to derive $D_i^*$.

\item The classifier may derive a clause that is structurally very
different from the original one (different attributes or number of
conditions). This is problematic in general, as it corresponds to a
larger-scale mistake in the query, which is a less likely scenario.

\item Classifiers try to avoid overfitting, which is problematic for
queries with high selectivity (e.g., single-tuple updates), as the
classifier is unlikely to generate any rules.

\end{itemize}


Therefore, while examining one query at a time superficially appears
to be a reasonable and efficient alternative, the reality is that one
has to model all constraints and transformations through the entire
log history. In the following section, we propose several
optimizations to our initial approach that make scaling to large data
and log sizes feasible. 


\iffalse
In this
section, we examine alternative, simpler models that process a single
query at a time, and demonstrate why they are insufficient.

\noindent
\textbf{WHERE repairs through classification:}
The \texttt{WHERE} clause of an update query is equivalent to a
rule-based binary classifier that splits tuples into two groups:
(1)~tuples that satisfy the conditions in the \texttt{WHERE} clause
and (2)~tuples that do not. Thus, by training a classifier,
such as decision trees \cite{quinlan1987} to learn
the correct classification rules rules for the \texttt{WHERE} clause.

\noindent
\textbf{SET repairs:}
This alternative approach constructs 
a simple linear system of equations to solve the parameters in the \texttt{SET}
when errors persist after fixing the \texttt{WHERE} clause:
For each expression in the \texttt{SET} clause we create a
linear equation, using unknown variables to represent any parameters
in the \texttt{SET} expression. 
  \begin{figure}[h]
  \centering
    \includegraphics[width = .6\columnwidth]{figures/heuristicacc}
    \vspace*{-.1in}
    \caption{Heuristic Approach vs. \sys on Single-Query. }
    \label{f:heuristic_acc} 
  \end{figure}
  \vspace*{-0.1in}
  
The na\"ive approach that we just described is heuristic in nature. It
is simple and fast, but it can only process a single incorrect query. As shown in
Figure~\ref{f:heuristic_acc}, the F-1 score of na\"ive heuristic approach is less 
than 0.6 while \sys maintain high accuracy in solving single query problem with
above 0.9 F-1 score across all database sizes. 
\fi


==> content/xx-heuristics.tex <==
\section{Heuristics}
\label{sec:heurstic}

\subsection{Attribute Slicing}

To further improve efficiency, we propose the attribute-slicing heuristic 
(Algorithm~\ref{alg:heu}) that may lose accuracy. This attribute-slicing
heuristic iteratively
generates the log repair by splitting the relevant 
attributes $Rel\mathcal{(A)}$ into
groups and fixing parameters involved 
in each group separately through a 
much smaller MILP problem. By 
controlling the number of attributes 
in each group, we bound the size of 
each MILP problem in the repair process.

\begin{algorithm}[htbp]
\caption{$AttributeSlicing$ heuristic.}
\label{alg:heu}
\begin{algorithmic}
\REQUIRE {$\mathcal{Q}, D_0, D_n, \mathcal{C}$}
\ENSURE {$\mathcal{Q^*}$}
\STATE $Rel\mathcal{(A)} \leftarrow FindRelAttr(\mathcal{Q}, D_n, \mathcal{C})$
\STATE $Rel\mathcal{(Q)} \leftarrow FindRelQuery(\mathcal{Q}, D_n, \mathcal{C})$
\STATE $\mathcal{G} \leftarrow SplitAttr(Rel\mathcal{(A)})$
\STATE $solved\_vals \leftarrow \emptyset$
\FOR {each $\partial (Rel\mathcal{(A)})$ in $\mathcal{G}$}
\STATE $\mathcal{Q'} \leftarrow PartialCF(\mathcal{Q}, \partial (Rel\mathcal{(A)}))$
\STATE $solved\_vals \leftarrow BasicApproach(\mathcal{Q'}, solved\_vals, ...)$
\ENDFOR
\STATE $\mathcal{Q}^* \leftarrow ConvertQLog(Q, solved\_vals)$
\STATE Return $\mathcal{Q}^*$
\end{algorithmic}
\end{algorithm}

In order to construct the sub MILP problem 
for a attribute group, we rewrite the conditional 
function, $f_q(t)$, into 
the partial conditional function format, $\partial (f_q(t))$.

\begin{definition} [Partial Conditional Function]
	The partial conditional function for a query $q$ over 
	attribute set $\partial(Rel\mathcal{(A)})$ is:
	\[
    \partial (f_q(t))= 
\begin{cases}
    \partial (f_{q.\mu} (t)) ,& \text{if } \partial (f_{q.\sigma} (t))\\
    t,              & \text{otherwise}
\end{cases}
\]
where
\begin{eqnarray*}
\partial (f_{q.\mu} (t)) &=& \{f|f\in f_{q.\mu}(t), \Pi_{f}(R) 
\in \partial (Rel\mathcal{(A)})\}\\
\partial (f_{q.\sigma} (t)) &=& \cup_{f \in f_{q.\sigma} (t)} \partial(f)
\end{eqnarray*}
Note that $\partial(f)$ is a transformation over a function 
(logical expression) $f$ defined
as following:
\[
\partial(f) = 
\begin{cases}
x,\ if\ \Pi_{f}(R) \cap \partial(Rel\mathcal{(A)}) = \emptyset\\
f, otherwise
\end{cases}
\]
$x$ is a newly introduced boolean variable. 
\end{definition} 
By doing so, we can easily construct the sub MILP problem 
in the same way as in the basic approach. Note that 
after each iteration, the solved variables, 
especially boolean variable $x$(s), are reused to provide 
constraint(s) for attributes that have not been examined. 
We demonstrate the process in Example~\ref{ex:heurstic}.

\begin{example}\label{ex:heurstic}
In this example, we demonstrate how to use Attribute-slicing heuristic to
solve the problem in Example~\ref{ex:taxes}. According to
Section~\ref{sec:opt}, we have:
\begin{eqnarray*}
\mathcal{F}(q_1) &=& \{rate, owed \} \\
\mathcal{F}(q_2) &=& \{owed\} \\
\mathcal{F}(q_3) &=& \{ID, rate, income, owed\}\\
Rel(\mathcal{A}) &=& \{ID, rate, income, owed\}
\end{eqnarray*}
Let us split the relevant attributes into groups: \\ 
$\{\{rate\}, \{owed\}, \{income\}, \{ID\}\}$.\\
Consider the first attribute group $\{rate\}$, we 
first rewrite the query log into $\partial(f_q(t))$ as the following:\\
\begin{minipage}{0.7\textwidth}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
            f_{q_1.\mu} &=& \{\{rate = 30\}\}; \\
f_{q_2.\mu} &=& \emptyset;  \\
f_{q_3.\mu} &=& \{\{rate = 25\}\};
        \end{align*}
    \end{minipage}
    \hspace{4em}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
           f_{q_1.\sigma} &=& x_1\\
            f_{q_2.\sigma} &=& true\\
           f_{q_1.\sigma} &=& x_3
        \end{align*}
    \end{minipage}
\end{minipage}

\smallskip

\indent We construct a sub MILP problem by linearizing
this query log over tuple $\{t_1, t_2, t_3, t_4\}$, parameterizing
the numeric variables, $30 and 25$, into $var1, var2$,
and setting the objective function as the minimum Euclidean
distance between modified numeric variable with original ones.
This sub MILP problem provides the following values: $var1 = 30, 
var2 = 25$;$t_1.x_1 = false, t_1.x_3 = false$; $ t_2.x_1 = true, 
t_2.x_3 = false$; $t_3.x_1 = false, t_3.x_3 = false$;
$t_4.x_1 = false; t_4.x_3 = true$.

\smallskip

In next iteration, we focus on attribute group $\{owed\}$ and find
the only numeric variable in $q_2$ should be $100$.
We then examine attribute group $\{income\}$, since we solved
$t_3.x_1 = false$ in the first iteration, the numeric 
variable $85700$ in the where clause of $q_1$ has to be 
changed into $86000+\epsilon$, where $\epsilon$
is a small number less than the minimum gap among values in
attribute $income$. Finally, we check attribute group
$\{ID\}$, and derive a log repair by revise $q_1$ as
\texttt{UPDATE Taxes Set rate = 30 WHERE income >= 86000+$\epsilon$ }. 
\end{example}








==> content/xx-impl.tex <==
\section{Implementation}

\sys is implemented as a Java-based middleware in front of PostgreSQL.

Talk about tricks to encode problem intto CPLEX/decision tree?




==> content/xx-related-full.tex <==

\section{Related Work}
\label{s:related} 
\sys tackles the problem of diagnosis and repair in relational query
histories (query logs). It does not aim to correct errors in the data
directly, but rather to find the underlying reason for reported errors
in the queries that operated on the data. This is in contrast to
traditional data 
cleaning~\cite{dallachiesa2013nadeef, rahm00, Raman01, Kalashnikov06, Fan2008b
} which focuses on identifying and correcting data
``in-place.'' Identifying and correcting errors is an important, and
rightfully well-studied problem. Existing literature has supplied a
variety of tools to capture errors originating from data
integration~\cite{Abiteboul99
},
recognizing the same entities in data~\cite{Koudas2006, GruenheidDS14
}, identifying true facts among conflicting
data~\cite{yin2008truth, DN09, ltm2012
}, and language support for
cleaning~\cite{Galhardas2000}. All of these techniques are
complimentary to our work. Their goal is to identify which data is
correct and which data is incorrect, but they don't look for the
sources of these errors in the processes or queries that generate and
modify this data. In fact the output of such methods can be used to
augment the complaint sets used by \sys, which focuses on identifying
errors in the queries that produced the data, rather than the data
itself.

An aspect of data cleaning focuses on providing repairs for the
identified errors~\cite{ChuIP13}. Tools in this domain have targeted
different methods and interactions for providing fixes, ranging from
functional dependencies~\cite{Fan2008b, ChuIP13
} and
rules~\cite{Beskales2010, Cong2007
} and functional
dependencies~\cite{Fan2008b, ChuIP13
}, to interactive methods that
solicit user feedback~\cite{Yakout, Raman01
}. As with the other data
cleaning approaches, all these techniques again operate on the data
directly. In contrast, \sys analyzes errors in the data to diagnose
and repair errors in queries that operated on the data. Thus, \sys
leverages the facts that some data errors are systemic, linked to
erroneous updates. Diagnosing the cause of the errors, will achieve
systematic fixes that will correct all relevant errors, even if they
have not been explicitly identified.

Closer to exploring systemic reasons and patterns for errors are
techniques such as Data Auditor~\cite{GolabKKS10, Golab2008
} and Data
X-Ray~\cite{wang2015}. Both tools tools identify features, which can
be selected from the tuple attributes, that best summarize or describe
groups of tuples (or specifically errors). While these tools can
generate feature sets or patterns of attributes that characterize
errors, these are not linked to the queries, but are again
characterizations over the data itself. Such techniques can be
tremendously useful if the processes that generate or modify the data
are unknown or black-box computations. In these cases, Data Auditor
and Data X-Ray can provide high-level clues for potential problems in
the data derivation process. However, both approaches are oblivious to
the actual queries that operated on the data, and they do not provide
particular fixes. Ontology-based why-not
explanations~\cite{tenCate2015} is very similar to Data X-Ray, but is
only relevant to absent tuples (deletions), and again does not
consider the query history.

The topic of query revisions has been studied in the context of
why-not explanations~\cite{Chapman2009}. These scenarios investigate
the absence of answers in a query result, and often attempt to modify
the query to change its outcome. Skyline
refinement~\cite{tran2010conquer} focuses specifically on refinements
that use skyline queries, while semi-automatic SQL
debugging~\cite{tzompanaki14semi} revises a given query to make it
return specified tuple groups in its output. All these approaches are
limited to selection predicates of \texttt{SELECT} queries, and they
only typically consider one query at a time. In contrast, \sys handles
update workloads, processes large query histories, and can model
several steps in the dataset's evolution.

Existing work on explaining query outputs~\cite{GebalyAGKS14} is also
limited in its applicability. The Scorpion system~\cite{Wu13}
processes a set of outlier points in an aggregate to identify
predicates on the input data as explanations. Roy and
Suciu~\cite{Roy2014} extended explanations with a formal framework
that handles complex SQL queries and database schemas involving
multiple relations and functional dependencies, but again their focus
is on \texttt{SELECT} workloads, rather than evolving datasets, and
they often target specific application domains~\cite{Khoussainova2012, Thirumuruganathan2012, Das2011, Fabbri2011, Bender14
}.

Finally, as \sys traces errors in the queries that manipulate data, it
has connections to the field of \emph{data and workflow provenance}.
our algorithms build on several formalisms introduced by work in this
domain. These formalisms express why a particular data item appears in
a query result, or how that query result was produced in relation to
input data~\cite{BunemanKT01,GKT07-semirings, CheneyCT09, CuiWW00
}.




==> content/xx-solutions-old.tex <==
\ewu{We don't talk about SET clauses anywhere. Are they trivial?  It's not obvious that conditional functions and linearizing them magically fix them.  Need to justify why we are focusing the text on WHERE clause range predicates}


\section{Basic Solution}

In this section we will introduce a simple approach to solve Prob-Complete.


Given $D'_n = C(D_n)$, able to roll back to fixed intermediate state $D'_i$.


\subsection{Metrics}

Metrics we use to measure how good a fix is.

Used in the optimization problem.




\subsection{Single-Query Case}

In this section, we walk through the core techniques in the case of a query sequence containing a single query.
\xxx{Walk through solution for each error type for each query type.}

Inserts and deletes are straight forward, however modifying WHERE clause is harder because
\xxx{why?}.  To deal with this challenge, we tried three algorithmic approaches.

\stitle{Constraint-solver (CPLEX)}
Describe how to encode problem as CPLEX

\stitle{Bounding Box}


\stitle{Decision Tree}
Describe how to encode as decision tree, what algorithm, and how to interpret learned tree.

Also, how to encode constraint that structure needs to be the same, by simply limiting the possible attribute
choices at each step in the learning algorithm.

\subsubsection{Comparing these approaches}

To understand the tradeoffs between these approachse, we ran a simple experiment for a single query.

Here are the results.


CPLEX takes the longest, however produces exact results.  However, it fails to produce any results if there are conflicting complaints.
Decision tree is fastest, however the quality of the results are poor.
Bounding box is similar to CPLEX in quality, however it generates results even if there are conflicting complaints.








\section{Prob-Complete}

Given the above, the algorithm for solving the complete complaint set problem is straightforward (Algorithm~\ref{alg:basic}).
We can simply try each query and return the one for which the best solution is found.

\subsection{Provenance-based Log Filtering}

Use provenance information (tuple-level or query level) to filter out queries that do not 
affect the complaint tuples at all.





\section{Incomplete Complaints}
\label{s:incomplete-algs}

Incomplete complaints are a challenge because the exesting algorithms fail.  We ran a simple experiment
where the complaint set contains only M\% of the true complaint set, and has N randomly generated erroneous complaints.
Figure~\ref{} shows that none of the algorithms work.

Describe assumptions for why a cleaning-based approach makes sense.

We use a cleaning-based method to deal with false positives, and some magic to deal with false negatives.

\subsection{False Positives}

Describe density, bi-partite graph, consistency, tuples affected scores.  Which ones work well, which ones don't.

NP-completeness of density-based approach.


\subsection{False Negatives}



\section{Multi-query Resolution}

We use a dynamic programming-based algorithm to support multiple queries.




\section{Rolling back the log}

background about why this is a hard problem

\subsection{A Solver-based approach}

Table $R(A,B)$ contains tuple $t_0=(a_0,b_0)$. Query $Q_1$ is applied to the
database: $Q_1 =$ UPDATE R SET $A=u_1$ WHERE $B\leq u_2$. The parameters $u_1$
and $u_2$ are constants specified by the query, but we parameterize them to
allow for their modification based on the complaints.

\smallskip

After the execution of $Q_1$, tuple $t_0$ has become $t_1=(a_1,b_1)$. We will
use attribute-level provenance to represent the resulting values $a_1$ and
$b_1$. For what follows, I use the linearization logic from section 4.4 of the
Tiresias paper.

\smallskip


Let $X$ be a Boolean variable that is true if the WHERE clause of $Q_1$
affects $t_0$: $X=(b_0\leq u_2)$. We will map this to integer variable $x$,
following the logic of the Tiresias provenance representation: $x\otimes
b_0\leq x\otimes u_2$.  We assign new, real variables $v_1= x\otimes
b_0$ and $v_2=x\otimes u_2$.

\smallskip

To linearize the expressions of $v_1$ and $v_2$, we use the following constraints (same as in Tiresias, page 8):

\begin{minipage}{0.7\textwidth}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
            &v_1\le b_0\\
            &v_1\le xM\\
            &v_1\ge b_0 - (1-x)M
        \end{align*}
    \end{minipage}
    \hspace{4em}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
            &v_2\le u_2\\
            &v_2\le xM\\
            &v_2\ge u_2 - (1-x)M
        \end{align*}
    \end{minipage}
\end{minipage}

\smallskip

Here, $M$ denotes a very large number (upper bound for the $u_i$).

\smallskip

In $t_1$ the attribute $a_1$ can be expressed: $a_1=x\otimes u_1 +
(1-x)\otimes a_0$, meaning that $a_1$ takes the value $u_1$ if $x=1$, and the
value $a_0$ if $x=0$.  We can now assign: $v_3= x\otimes
u_1$ and $v_4=(1-x)\otimes a_0$, and similarly linearize them:

\begin{minipage}{0.7\textwidth}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
            &v_3\le u_1\\
            &v_3\le xM\\
            &v_3\ge u_1 - (1-x)M
        \end{align*}
    \end{minipage}
    \hspace{4em}
    \begin{minipage}[t]{0.2\textwidth}
        \begin{align*}
            &v_4\le a_0\\
            &v_4\le (1-x)M\\
            &v_4\ge a_0 - xM
        \end{align*}
    \end{minipage}
\end{minipage}

So, now, we can express the transformation of $t_0$ through query $Q_1$ with a
program with 1 integer variable ($x$) and 8 real variables ($u_1$, $u_2$,
$v_1$, $v_2$, $v_3$, $v_4$, $a_1$, $b_1$). $a_0$ and $b_0$ are constants in
this case, as they are the original values of $t_0$, but they could also be
variables if $t_0$ was derived from another query.

Overall, we have a mixed integer program with the constraints:
\begin{align*}
    &b_1=b_0\\
    &a_1 = v_3+v_4\\
    &0\leq x\leq 1\\
    &v_1\le b_0\\
    &v_1\le xM\\
    &v_1\ge b_0 - (1-x)M\\
    &v_2\le u_2\\
    &v_2\le xM\\
    &v_2\ge u_2 - (1-x)M\\
    &v_3\le u_1\\
    &v_3\le xM\\
    &v_3\ge u_1 - (1-x)M\\
    &v_4\le a_0\\
    &v_4\le (1-x)M\\
    &v_4\ge a_0 - xM
\end{align*}

\smallskip 

This is for the transformation of a single tuple ($t_0$) by a single query.
Similar constraints would be derived for the other tuples, and other queries.
In the end, based on the complaints, we can assign values to the corresponding
variables (e.g., $a_1=5$), and solve the program for the parameters $u_i$,
which will give us a correction. The optimization objective can be set so that
the sum of the differences from the query parameters is minimized.

\smallskip

Since the provenance maintains the transformations, there wouldn't be a need
for rolling back the database instance.



\subsection{Hybrid algorithm}

Describe Exhastive and greedy special cases.


Algorithm:

\begin{verbatim}

querylog = filter(querylog)
batchsize = 1
while i > 0
  batch = [qi to q{i-batchsize}]
  alexandras_solver(batch)
  i -= batchsize

\end{verbatim}


==> content/xx-usecase.tex <==

\section{Real-world examples}
\label{s:usecase}

\alex{I am not convinced that these deserve a section.  It would make sense if we actually applied our system on them and had something to say about the derived diagnoses and fixes.  As they are, I would use as examples in the introduction instead.}

\subsection{Telco}

Call centers get customer complaints about billing all the time.
For example, there was a change in the tax law, but the transactions
that updated the taxes didn't change, so they would get lots of
customer complaints.  Each customer agent usually fixes each problem
individually, however, it's a system problem to all of Kansas that
usually doesn't get caught until late in the game.  In this case
it's a faulty update to a numerical value whose effects compound
over time.  There is external domain knowledge to isolate the
culprits to tax-related transactions, and sensitivity analysis can
be useful.

\subsection{Insurance}

A colleague recently switched to medicare but because of a problem
with the transactions to switch him from his previous to new
insurance, it's caused him 6 months of headaches.  3 months ago he
learned that a bunch of other people have been complaining about
the same issues regarding the switch.  In this case it's a categorical
change (from one insurance to another) that has more obvious impact.




==> hacks.tex <==


